A combinatorial description of the LOSS Legendrian knot invariant

In this note, we observe that the hat version of the Heegaard Floer invariant of Legendrian knots in contact three-manifolds defined by Lisca-Ozsvath-Stipsicz-Szabo can be combinatorially computed. We rely on Plamenevskaya's combinatorial description of the Heegaard Floer contact invariant.

==> Combinatorial LOSS arxiv v1/commands.tex <==
% Roman number for equation
\renewcommand{\theequation}{\roman{equation}}


% THEOREMS
\theoremstyle{definition}
\newtheorem{theorem}{{Theorem}}[section]
\newtheorem{lemma}[theorem]{{Lemma}}
\newtheorem{proposition}[theorem]{{Proposition}}
\newtheorem{definition}[theorem]{{Definition}}
\newtheorem{corollary}[theorem]{{Corollary}}
\newtheorem{example}[theorem]{{Example}}
\newtheorem{conjecture}[theorem]{{Conjecture}}
\newtheorem{remark}[theorem]{{Remark}}
\newtheorem{claim}[theorem]{{Claim}}
\newtheorem{question}[theorem]{Question}



% COMMON RINGS
\newcommand{\C}{\mathbb{C}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\F}{\mathbb{F}}






\newcommand{\CFK}{\textit{CFK}} 
\newcommand{\cfhat}{\widehat{\textit{CF}}}
\newcommand{\hfhat}{\widehat{\textit{HF}}}
\newcommand{\HFKhat}{\widehat{\textit{HFK}}}
\newcommand{\HFKminus}{\textit{HFK}^{-}}
\newcommand{\lossminus}{\mathfrak{L}(L)}
\newcommand{\loss}{\widehat{\mathfrak{L}}}
\newcommand{\lossl}{\widehat{\mathfrak{L}}(L)}


\newcommand{\s}{\mathfrak{s}}

\newcommand{\cc}{\mathbf{c}}
\newcommand{\yy}{\mathbf{y}}

\newcommand{\xx}{\mathbf{x}}
\newcommand{\ob}{\mathfrak{ob}}


